SustainBench: Benchmarks for Monitoring the Sustainable Development Goals with Machine Learning

Progress toward the United Nations Sustainable Development Goals (SDGs) has been hindered by a lack of data on key environmental and socioeconomic indicators, which historically have come from ground surveys with sparse temporal and spatial coverage. Recent advances in machine learning have made it possible to utilize abundant, frequently-updated, and globally available data, such as from satellites or social media, to provide insights into progress toward SDGs. Despite promising early results, approaches to using such data for SDG measurement thus far have largely evaluated on different datasets or used inconsistent evaluation metrics, making it hard to understand whether performance is improving and where additional research would be most fruitful. Furthermore, processing satellite and ground survey data requires domain knowledge that many in the machine learning community lack. In this paper, we introduce SustainBench, a collection of 15 benchmark tasks across 7 SDGs, including tasks related to economic development, agriculture, health, education, water and sanitation, climate action, and life on land. Datasets for 11 of the 15 tasks are released publicly for the first time. Our goals for SustainBench are to (1) lower the barriers to entry for the machine learning community to contribute to measuring and achieving the SDGs; (2) provide standard benchmarks for evaluating machine learning models on tasks across a variety of SDGs; and (3) encourage the development of novel machine learning methods where improved model performance facilitates progress towards the SDGs.

==> 06_checklist.tex <==
\newpage
\section*{Checklist}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
     \answerYes{}
  \item Did you describe the limitations of your work?
     \answerYes{In \Cref{sec:discussion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{In \Cref{sec:discussion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}. URLs to our Google Drive data folder and our GitHub code repo are in the \Cref{app:dataset_storage_plans}.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \Cref{app:baseline_models}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{We report baseline results from existing papers.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{We report baseline results from existing papers.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{In \Cref{app:sec:dataset}}
  \item Did you mention the license of the assets?
    \answerYes{In \Cref{app:sec:licenses}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{In \Cref{app:dataset_storage_plans}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{In \Cref{app:sec:licenses}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}. The data does not contain personally identifiable information or offensive content. See \Cref{sec:discussion} for a discussion on privacy concerns and how the geocoordinates in the survey-derived data is intentionally randomly jittered to protect privacy.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}. No crowdsourcing or human subjects were involved.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}



==> instruction.tex <==
\section{Appendix Guidelines}

Include extra information in the appendix. This section will often be part of the supplemental material. Please see the call on the NeurIPS website for links to additional guides on dataset publication.

\begin{enumerate}

\item Submission introducing new datasets must include the following in the supplementary materials:
\begin{enumerate}
  \item Dataset documentation and intended uses. Recommended documentation frameworks include datasheets for datasets, dataset nutrition labels, data statements for NLP, and accountability frameworks.
  \item URL to website/platform where the dataset/benchmark can be viewed and downloaded by the reviewers.
  \item Author statement that they bear all responsibility in case of violation of rights, etc., and confirmation of the data license.
  \item Hosting, licensing, and maintenance plan. The choice of hosting platform is yours, as long as you ensure access to the data (possibly through a curated interface) and will provide the necessary maintenance.
\end{enumerate}

\item To ensure accessibility, the supplementary materials for datasets must include the following:
\begin{enumerate}
  \item Links to access the dataset and its metadata. This can be hidden upon submission if the dataset is not yet publicly available but must be added in the camera-ready version. In select cases, e.g when the data can only be released at a later date, this can be added afterward. Simulation environments should link to (open source) code repositories.
  \item The dataset itself should ideally use an open and widely used data format. Provide a detailed explanation on how the dataset can be read. For simulation environments, use existing frameworks or explain how they can be used.
  \item Long-term preservation: It must be clear that the dataset will be available for a long time, either by uploading to a data repository or by explaining how the authors themselves will ensure this.
  \item Explicit license: Authors must choose a license, ideally a CC license for datasets, or an open source license for code (e.g. RL environments).
  \item Add structured metadata to a dataset's meta-data page using Web standards (like schema.org and DCAT): This allows it to be discovered and organized by anyone. If you use an existing data repository, this is often done automatically.
  \item Highly recommended: a persistent dereferenceable identifier (e.g. a DOI minted by a data repository or a prefix on identifiers.org) for datasets, or a code repository (e.g. GitHub, GitLab,...) for code. If this is not possible or useful, please explain why.
\end{enumerate}

\item For benchmarks, the supplementary materials must ensure that all results are easily reproducible. Where possible, use a reproducibility framework such as the ML reproducibility checklist, or otherwise guarantee that all results can be easily reproduced, i.e. all necessary datasets, code, and evaluation procedures must be accessible and documented.

\item For papers introducing best practices in creating or curating datasets and benchmarks, the above supplementary materials are not required.
\end{enumerate}




\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone.

\subsection{Citations within the text}

The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.

The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{https://urldefense.com/v3/__http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf__;!!GX6Nv3_Pjr8b-17qtCok029Ok438DqXQ!l-erlUAeEokZ3h7n56lTM5dpI0saUi0X4hdZFLDJEpXTsfAw4H9Y3NsZPvhF$ }
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}

If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2021+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}

If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2021}
\end{verbatim}

As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous.''

\subsection{Footnotes}

Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).

Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}

\subsection{Figures}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.

You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.

\subsection{Tables}

All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://urldefense.com/v3/__https://www.ctan.org/pkg/booktabs__;!!GX6Nv3_Pjr8b-17qtCok029Ok438DqXQ!l-erlUAeEokZ3h7n56lTM5dpI0saUi0X4hdZFLDJEpXTsfAw4H9Y3NdoMrBm$ }
\end{center}
This package was used to typeset Table~\ref{sample-table}.

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}


\section{Final instructions}

\subsection{Suppressing line numbers in supplementary materials}
If you need to suppress line numbers in the supplementary materials because 
they interfere with the text, for instance because you are including a 
data sheet in 2-column format, you can do so by
placing the following command before it:
\begin{verbatim}
    \let\linenumbers\nolinenumbers\nolinenumbers
\end{verbatim}


==> zOLD_01_intro.tex <==
\section{Introduction}

In 2015, the United Nations (UN) set the Sustainable Development Goals (SDGs) as a call to action for all countries to promote prosperity while protecting the planet~\cite{2015transforming}. Proposed as targets to be achieved by 2030, the SDGs are 17 interrelated goals that span social, economic, and environmental spheres; they range from ending poverty to achieving gender equality to combating climate change. To make the SDGs more actionable, the goals were further expanded into 169 Targets and 247 Indicators that elaborate on specific SDG components and ways of measuring progress toward each goal. A full list of the 17 SDGs, their descriptions, and corresponding targets and indicators can be found in \Cref{app:tab:sdgs_full} of the Appendix.

So important and so uncontroversial are the SDGs that all countries on Earth have agreed to work toward them. 
In order to meet objectives, however, countries first have to know their starting point and rate of progress. Broadly speaking, there are two ways the SDGs can be monitored. The first, traditional way is through official statistics collected by civil registrations, population-based surveys and censuses, and specialized studies. Collecting official statistics is itself a major challenge, especially in low-income countries. As outlined in the initial Global Sustainable Development Report (GSDR), traditional ways of measuring progress (i.e. surveys) share a number of serious shortcomings \cite{gsdr2014}. First, official statistics are expensive and require a high level of statistical capacity in all countries. Despite decades of international statistical support, many poor countries continue to lack the resources and capacity to carry out surveys. 
Second, official statistics are collected for provinces/states and lack the spatial disaggregation needed to analyze trends and trade-offs at the local level. Important statistics like GDP and crop production are shared with the UN at the national level, potentially obscuring subnational patterns in productivity. Third, surveys are conducted at most annually and often every few years or less. As a result, the statistics cannot be used as early warnings for events like food crises or disease outbreaks. Lastly, it has been argued that sustainability can only be achieved locally, and traditional data-acquisition, with its spatial and temporal coarseness, will never yield insights on why some policies and actions are successful while others are not \cite{xu2020assessing}. \chenlin{consider moving this paragraph to appendix?}

In light of these shortcomings, the GSDR report concluded that ``it is highly unlikely that comprehensive, high-quality data for traditional progress indicators will be available for all (or even most) countries within the next 20 years'' \cite{gsdr2014}.
Today, six years after the unveiling of the SDGs, many gaps indeed still exist in monitoring progress. Official tracking of data availability is conducted by the UN Statistical Commission, which classifies each indicator into one of three tiers: indicator is well-defined and data are regularly produced by at least 50\% of countries (Tier I), indicator is well-defined but data are not regularly produced by countries (Tier II), and the indicator is currently not well-defined (Tier III). As of the latest report from March 2021, 136 indicators have regular data from at least 50\% of countries, 107 indicators have sporadic data, and 4 indicators are a mix depending on the data of interest (\Cref{app:tab:sdgs_full}) (cite). For example, for monitoring global poverty (SDG 1), the proportion of a country's population living below the international poverty line (Indicator 1.1.1) is reported annually for all countries, but the economic loss attributed to natural and man-made disasters (Indicator 1.5.2) is only sparsely documented. \chenlin{consider moving this paragraph to appendix?}

Fortunately, other sources of data relevant to monitoring the SDGs have become abundant in the last two decades, offering a second way of tracking progress referred to by the UN as the ``big data approach''. Data like satellite imagery, social media posts, and mobile phone activity are growing in volume every year as more satellites launch into space and more people around the world connect to the internet (cite). These non-traditional datasets do not possess the shortcomings present in surveys: they are available at low marginal cost, capture information at disaggregated spatial resolutions, generate real-time updates, and offer continuous or near-continuous temporal resolution. 
Researchers have demonstrated how nighttime lights \cite{jean2016combining}, residential footprints \cite{huang2021using}, and mobile phone data \cite{blumenstock2015predicting} can estimate wealth at high spatial resolution; multi-spectral satellite imagery can map annual land cover \cite{friedl2002global,buchhorn2020copernicus}, deforestation \cite{hansen2013high}, agricultural diversity \cite{cdl,wang2020mapping}, and crop yields \cite{azzari2017towards, you2017deep}; and how satellite and social media data can localize natural disasters in real-time \cite{debruijin2019a} as well as elucidate the effects of climate change on disasters over decades \cite{tellman2021satellite}. \chenlin{consider merge with the next paragraph? and introduce machine learning has made it possible to use new data sources}

Underpinning much of the success in using non-traditional datasets are advances in machine learning, especially in neural networks that allow knowledge to be extracted from unstructured data. For instance, Jean \emph{et al.} (2016) used transfer learning to map poverty across Africa \cite{jean2016combining, yeh2020using}, Huang \emph{et al.} (2021) used a Mask-RCNN to extract building footprints to evaluate the impact of an anti-poverty program \cite{huang2021using}, and Lee \emph{et al.} (2021) combined image classification with class activation maps to locate illegal, highly-polluting brick kilns in Bangladesh \cite{lee2021scalable}.
For the most part, methods used so far have been adapted from methods originally designed for and validated on canonical deep learning datasets (e.g. ImageNet), but the datasets and tasks relevant to SDG monitoring are unique enough to merit their own methodology.
To start, gaps in monitoring SDGs are widest in low-income countries, where only sparse ground labels are available to train or validate predictive models, so the best-performing methods are likely to take advantage of massive unlabeled data, labels out-of-domain, and sparse or low-quality labels in-domain. Satellite imagery is also unique in its underlying geographic structure, which can be leveraged to learn feature representations \cite{jean2019tile2vec}. Lastly, multiple input modalities (e.g. satellite imagery and cell phone records) can be combined to achieve better predictions than single-stream inputs \cite{chi2021microestimates}, but the best way to do so is still unknown.

Currently, methodological progress on the ``big data approach'' to monitoring SDGs is hindered by at least three challenges. First, labeled data at fine spatial scales are difficult to come by.\chenlin{do not see how our dataset benchmark solve this issue} For some indicators, labels do not exist at all. When they do exist, ground labels are distributed across academic research groups, non-profits, and companies, or, when labels are public, locating them requires navigating government and NGO websites. Second, downloading and working with satellite imagery requires domain knowledge that many in the machine learning community lack. \chenlin{this point looks convincing}Satellite imagery can include multiple bands along the electromagnetic spectrum; are supplied by sensors spanning centimeter to kilometer resolution, and require geospatial software to remove clouds and coregister with labels. Third, approaches have been evaluated on different datasets, data splits, or evaluation metrics, \chenlin{this point looks convincing}making it hard to understand whether performance is improving and where additional work would be most fruitful. This is in stark contrast to canonical machine learning datasets like MNIST, CIFAR-10, and ImageNet that have standardized inputs, outputs, and evaluation criteria and have therefore facilitated the development of computer vision algorithms.

The purpose of this paper is to introduce the machine learning community to the challenges of monitoring SDGs and present \textsc{SustainBench}, a compilation of datasets and benchmarks for monitoring the SDGs with machine learning.
Our goal is to 
\begin{itemize}
    \item [a)] Lower the barriers to entry by supplying satellite imagery and other inputs.
    \item [b)] Provide benchmarks to standardize evaluation on these important tasks and potentially draw attention from the community to these tasks.
\end{itemize}

In this first version of \textsc{SustainBench}, we cover seven SDGs across [x] datasets: No Poverty (SDG 1), Zero Hunger (SDG 2), Good Health and Well-being (SDG 3), Quality Education (SDG 4), Clean Water and Sanitation (SDG 6), Climate Action (SDG 13), and Life on Land (SDG 15). Most results have been published previously and some datasets have been made public; however, this is the first time that data splits have been standardized to enable benchmarking. In compiling the dataset, we prioritized data with high resolution ground truth in low-income countries, where monitoring with non-traditional data sources is most urgently needed. When ground truth in low-income countries is unavailable, we provide inputs and outputs in high- or middle-income countries that simulate the low-income setting (e.g. weak labels, few labels) to validate new methods.

The remainder of this paper is organized as follows. Section \ref{sec:related} provides a survey of related datasets; Section \ref{sec:data} introduces the SDGs and datasets currently covered by \textsc{SustainBench} and where methodological advances are needed; Section \ref{sec:benchmarks} reports the current state-of-the-art performance on each dataset; and Section \ref{sec:discussion} discusses the limitations and future directions of this work. 
Detailed information about the inputs, outputs, and tasks for each dataset can be found in the Appendix.


\definecolor{rowcolor}{rgb}{0.88,1,1}
\begin{table}[ht]
\centering
\caption{The UN Sustainable Development Goals (SDGs) with datasets in \textsc{SustainBench}, along with the classification of their indicators and current \textsc{SustainBench} coverage. we defined indicators in the intro.
}
\label{tab:sdgs}
\begin{adjustbox}{max width=0.99\linewidth}
\begin{tabular}{cp{0.18\textwidth}p{0.33\textwidth}cccc}
    \toprule
    \textbf{SDG} & \textbf{Name} & \textbf{Description} & \multicolumn{3}{c}{\textbf{\# Indicators}} & \textbf{\# \textsc{SustainBench}} \\
    \cline{4-6}
    \textbf{\#} & & & Tier I & Tier II & Tier I/II & \textbf{Datasets} \\
    \midrule
    1 & No Poverty & End poverty in all its forms everywhere & 5 & 8 & 0 & 2 \\
    2 & Zero Hunger & End hunger, achieve food security and improved nutrition and promote sustainable agriculture & 10 & 4 & 0 & 5 \\
    3 & Good Health and Well-Being & Ensure healthy lives and promote well-being for all at all ages & 25 & 3 & 0 & 2 \\
    4 & Quality Education & Ensure inclusive and quality education for all and promote lifelong learning & 5 & 6 & 1 & 1 \\
    6 & Clean Water and Sanitation & Ensure access to water and sanitation for all & 7 & 4 & 0 & 1 \\
    13 & Climate Action & Take urgent action to combat climate change and its impacts & 2 & 6 & 0 & 1 \\
    15 & Life on Land & Sustainably manage forests, combat desertification, halt and reverse land degradation, halt biodiversity loss & 11 & 2 & 1 & 2 \\
    \midrule
    & & & & & \textbf{Total} & 14 \\
    \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}



==> zOLD_01_intro_edited.tex <==
\section{Introduction}

\chris{Highlight how much work that goes into preparing this dataset}
\chris{Condense SDGs}

\chris{We need something like the following:

In this paper, we present a curated suite of 14 benchmark tasks spanning 7 SDGs. These benchmarks are not only valuable to improving sustainability measurements but also offer machine learning challenges. XX tasks involve multi-modal data street-view + Satellites. YY tasks have multi-task learning. ZZ tasks require self-supervision.

The use of machine learning tools to do this analysis is of high interest to the UN (cite some UN publication that uses related models). This underscores the real-world value of providing this benchmark.

Explain the value-add of gathering these datasets in a uniform benchmark, even though we are ``re-using'' a number of existing datasets. Think about how we could persuade reviewers even if we didn't have new datasets.

1. real-world stakeholders (UNDP, World Bank) are interested (cite!)

2. lots of work - hand-labeled data (brick kilns), satellite image projections, matching street-level with satellite geocoordinates, data cleaning

3. unique challenges for ML community
}

In 2015, the United Nations (UN) set the Sustainable Development Goals (SDGs) as a call to action for all countries to promote prosperity while protecting the planet~\cite{2015transforming}. Proposed as targets to be achieved by 2030, the SDGs are 17 interrelated goals that span social, economic, and environmental spheres; they range from ending poverty to achieving gender equality to combating climate change. 
A full list of the 17 SDGs, their descriptions, and more detailed targets and indicators can be found in \Cref{app:tab:sdgs_full} of the Appendix.

In order to meet objectives, countries first have to know their starting point and rate of progress. 
Progress towards SDGs is traditionally monitored through statistics collected by civil registrations, population-based surveys and censuses, and specialized studies~\cite{??}. Unfortunately, collecting official statistics is itself a major challenge, as
surveys are expensive and require a high level of statistical capacity ~\cite{gsdr2014}. 
As a result, only 55\% of SDG indicators have regular data from more than half of the world's countries, while 43\% of indicators have sporadic data (2\% are a mix depending on the data of interest) (\Cref{app:tab:sdgs_full}) (cite).
Furthermore, official statistics are reported at the province/state or national level annually or every few years, obscuring fine-grained trends across space and time.
It has been argued that sustainability is achieved locally, and traditional data acquisition at coarse scales will rarely yield insights on why some policies and actions are successful while others are not \cite{xu2020assessing}.


Fortunately, other sources of data relevant to monitoring the SDGs have become abundant in the last two decades, offering a second way of tracking progress referred to by the UN as the ``big data approach'' \cite{gsdr2014}. Data like satellite imagery, social media posts, and mobile phone activity are growing in volume every year as more satellites launch into space and more people around the world connect to the internet (cite). Although these non-traditional datasets typically only provide indirect measurements of SDG indicators, they do not possess the shortcomings present in surveys: they are available at low marginal cost, capture information at disaggregated spatial resolutions, generate real-time updates, and offer continuous or near-continuous temporal resolution.
\se{consider adding a sentence connecting these two paragraphs and motivate ML ( these datasets provide indirect/noisy measurements of the indicators of interest) }

Recent advances in machine learning have made it possible to use these non-traditional datasets for monitoring and enabling progress toward the SDGs. Researchers have demonstrated how, using machine learning, nighttime lights \cite{jean2016combining}, residential footprints \cite{huang2021using}, and mobile phone data \cite{blumenstock2015predicting} can estimate poverty at high spatial resolution (SDG 1);
\se{might not be obvious why wealth is related to the SDGs. maybe better to mention poverty and SDG1}
multi-spectral satellite imagery can map annual land cover \cite{friedl2002global,buchhorn2020copernicus}, deforestation \cite{hansen2013high}, agricultural diversity \cite{cdl,wang2020mapping}, and crop yields \cite{azzari2017towards, you2017deep} (SDG 2); and how satellite and social media data can localize natural disasters in real-time \cite{debruijin2019a} as well as elucidate the effects of climate change on disasters over decades \cite{tellman2021satellite}. \se{same for the rest. i think we should make the connection to SDG more explicit for readers not familiar with them}

For the most part, methods used so far have been adapted from methods originally designed for and validated on canonical deep learning datasets (e.g. ImageNet), but the datasets and tasks relevant to SDG monitoring are unique enough to merit their own methodology.
For example, gaps in monitoring SDGs are widest in low-income countries, where only sparse ground labels are available to train or validate predictive models. The best-performing methods are likely to take advantage of massive unlabeled data, labels out-of-domain, and sparse or low-quality labels in-domain.
\se{could also mention the domain shift issue: e.g. models trained to recognize objects on imagenet won't work on photos in developing world (see Does Object Recognition Work for Everyone?)}

Currently, methodological progress on the ``big data approach'' to monitoring SDGs is hindered by the following  challenges. 
First, downloading and working with satellite imagery, development surveys, etc. 
requires domain knowledge that many in the machine learning community lack. 
Second, approaches have been evaluated on different datasets, data splits, or evaluation metrics, making it hard to understand whether performance is improving and where additional work would be most fruitful. This is in stark contrast to canonical machine learning datasets like MNIST, CIFAR-10~\cite{krizhevsky2009learning}, and ImageNet~\cite{ILSVRC15} that have standardized inputs, outputs, and evaluation criteria and have therefore facilitated the development of machine learning algorithms~\cite{?}.


To facilitate methodological progress, this paper presents \textsc{SustainBench}, a compilation of datasets and benchmarks for monitoring the SDGs with machine learning.
Our goals are to 
\begin{enumerate}
    \item lower the barriers to entry by supplying domain-specific datasets in development economics and environmental science,
    \item provide benchmarks to standardize evaluation on tasks related to SDG monitoring, and
    \item encourage the machine learning community to evaluate relevant methods on problems of global significance and develop methods specifically for monitoring the SDGs.
\end{enumerate}

In \textsc{SustainBench}, we curate a suite of 14 benchmarks across 7 SDGs: No Poverty (SDG 1), Zero Hunger (SDG 2), Good Health and Well-being (SDG 3), Quality Education (SDG 4), Clean Water and Sanitation (SDG 6), Climate Action (SDG 13), and Life on Land (SDG 15). Most results have been published previously and some datasets have been made public; however, this is the first time that data splits have been standardized to enable benchmarking. We also summarize the performance of baseline models on each task from prior work.


The remainder of this paper is organized as follows. Section \ref{sec:related} provides a survey of related datasets; Section \ref{sec:data} introduces the SDGs and datasets currently covered by \textsc{SustainBench} and where methodological advances are needed; Section \ref{sec:benchmarks} reports the current state-of-the-art performance on each dataset; and Section \ref{sec:discussion} discusses the limitations and future directions of this work. 
Detailed information about the inputs, outputs, and tasks for each dataset can be found in the Appendix.


\definecolor{rowcolor}{rgb}{0.88,1,1}
\begin{figure}[h]
\centering
\begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{figures/figure1.png}
\end{subfigure}
\vfill
\begin{subfigure}[b]{\linewidth}
\begin{adjustbox}{max width=0.99\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{0.2\textwidth}p{0.35\textwidth}ccc}
    \toprule
    \textbf{SDG Name}  & \textbf{Task} & \textbf{Input$\to$ Output} & \textbf{\# examples} & \textbf{Metric} \\
    \midrule
    \multirow{2}{*}{1. No Poverty} &  Poverty prediction over space~\cite{yeh2020using} & Satellite imagery $\to$ Poverty indices & &\multirow{2}{*}{$R^2$}  \\
     &   Poverty prediction over time~\cite{yeh2020using} & Satellite imagery $\to$ Poverty indices &  & \\
     \midrule
    2. Zero Hunger &  Cropland classification~\cite{wang2020weakly} & Satellite imagery $\to$ Cropland or not & &Acc  \\
    & Crop type classification~\cite{rustowicz2019semantic} & Satellite imagery $\to$ Crop type &  &  \\
    &  Crop yield regression & Satellite histograms $\to$ County-level yields &  & \cite{you2017deep,wang2018transfer} \\
     & Farmland parcel delineation~\cite{aung2020farm} & Satellite imagery $\to$ Field boundaries & 1,966 &\cite{aung2020farm} \\
    \midrule
    3. Good Health and Well-being &  &    &  \\
    \midrule
    4. Quality Education &  &  &    \\
    \midrule
    6. Clean Water and Sanitation &  &    &  \\
    \midrule
    13. Climate Action & Brick kiln detection &  &  &  \\
    \midrule
    15. Life on Land & Representation learning for land cover~\cite{jean2019tile2vec} &  &  &   \cite{jean2019tile2vec} \\
    & Out-of-domain land cover classification~\cite{wang2020meta} & & & \cite{wang2020meta} \\
    \bottomrule
\end{tabular}
\end{adjustbox}
\end{subfigure}
\caption{The UN Sustainable Development Goals (SDGs) with datasets in \textsc{SustainBench}, along with the classification of their indicators and current \textsc{SustainBench} coverage.
}
\label{tab:sdgs}
\end{figure}

==> zOLD_datasets.tex <==













